Settling Time vs. Accuracy Tradeoffs for Clustering Big Data

We study the theoretical and practical runtime limits of k-means and k-median clustering on large datasets. Since effectively all clustering methods are slower than the time it takes to read the dataset, the fastest approach is to quickly compress the data and perform the clustering on the compressed representation. Unfortunately, there is no universal best choice for compressing the number of points - while random sampling runs in sublinear time and coresets provide theoretical guarantees, the former does not enforce accuracy while the latter is too slow as the numbers of points and clusters grow. Indeed, it has been conjectured that any sensitivity-based coreset construction requires super-linear time in the dataset size. We examine this relationship by first showing that there does exist an algorithm that obtains coresets via sensitivity sampling in effectively linear time - within log-factors of the time it takes to read the data. Any approach that significantly improves on this must then resort to practical heuristics, leading us to consider the spectrum of sampling strategies across both real and artificial datasets in the static and streaming settings. Through this, we show the conditions in which coresets are necessary for preserving cluster validity as well as the settings in which faster, cruder sampling strategies are sufficient. As a result, we provide a comprehensive theoretical and practical blueprint for effective clustering regardless of data size. Our code is publicly available and has scripts to recreate the experiments.

==> tables/composition.tex <==
\begin{table*}
    \centering
    \tiny
    \begin{tabular}{|c|cc|cc|cc|cc|}
        \hline
        & \multicolumn{8}{c|}{Method} \\
        \cline{2-9} & \multicolumn{2}{c|}{Uniform Sampling} & \multicolumn{2}{c|}{Lightweight} & \multicolumn{2}{c|}{Welterweight} & \multicolumn{2}{c|}{Fast Coreset} \\
        & Streaming & Static & Streaming & Static & Streaming & Static & Streaming & Static \\
        \cline{2-9}
        $c$-outlier & 221 $\pm$ 15K & 261 $\pm$ 44K & 1.07 $\pm$ 0.0 & 5.51 $\pm$ 78.9 & 1.09 $\pm$ 0.0 & 12.1 $\pm$ 80.1 & 1.13 $\pm$ 0.0 & 1.11 $\pm$
        0.0 \\
        Geometric & 66.5 $\pm$ 2.7K & 140 $\pm$ 1.8K & 85.2 $\pm$ 2.8K & 45.6 $\pm$ 4.2K & 1.09 $\pm$ 0.0 & 10.4 $\pm$ 349 & 1.15 $\pm$ 0.0 & 1.12 $\pm$ 0.0 \\
        Gaussian Mix. & 1.51 $\pm$ 0.07 & 2.42 $\pm$ 2.52 & 2.35 $\pm$ 0.67 & 2.38 $\pm$ 1.78 & 1.45 $\pm$ 0.05 & 3.65 $\pm$ 3.85 & 1.15 $\pm$ 0.0 & 1.24 $\pm$
        0.0 \\
        Benchmark & 1.10 $\pm$ 0.0 & 1.07 $\pm$ 0.0 & 1.08 $\pm$ 0.0 & 1.11 $\pm$ 0.0 & 1.09 $\pm$ 0.0 & 1.11 $\pm$ 0.0 & 1.18 $\pm$ 0.0 & 1.16 $\pm$ 0.0 \\
        MNIST & 1.42 $\pm$ 0.0 & 1.08 $\pm$ 0.0 & 1.07 $\pm$ 0.0 & 1.07 $\pm$ 0.0 & 1.02 $\pm$ 0.0 & 1.09 $\pm$ 0.0 & 1.12 $\pm$ 0.0 & 1.08 $\pm$ 0.0 \\
        Adult & 1.33 $\pm$ 0.0 & 895K $\pm$ 3.2B & 1.09 $\pm$ 0.0 & 1.09 $\pm$ 0.0 & 1.27 $\pm$ 0.01 & 1.32 $\pm$ 0.0 & 1.14 $\pm$ 0.0 & 1.15 $\pm$ 0.0 \\
        \hline
    \end{tabular}
    \caption{Distortion means and variances in the streaming and non-streaming setting for each method. We default to $m=20k$.}
    \label{tbl:composition}
\end{table*}



==> tables/lloyds.tex <==
\begin{table}
    \centering
    \small
    \begin{tabular}{|c|cccc|}
        \hline
        & \makecell{Uniform \\ Sampling} & Lightweight & Welterweight & \makecell{Fast \\ Coreset} \\
        MNIST & 12450 & 12379 & 12512 & 12449 \\
        Adult & 24982 & 24935 & 24944 & 25013 \\
        Song & 16753 & 16612 & 16950 & 17010 \\
        Census & 36697 & 35577 & 37379 & 32163 \\
        Cover-Type & 10506 & 10337 & 10032 & 9787 \\
        \hline
    \end{tabular}
    \caption{$cost(P, \calC_S)$, where $P$ is the whole dataset and $\calC_S$ is found via Lloyd's algorithm on the coreset. Sample sizes down the rows are
    $m=4K,4K,20K,20K,20K$ and initializations are identical within each row. We only show the first 5 digits of the cost for readability.}
    \label{tbl:lloyds}
\end{table}


